Nominal Cellular Automata

The emerging field of Nominal Computation Theory is concerned with the theory of Nominal Sets and its applications to Computer Science. We investigate here the impact of nominal sets on the definition of Cellular Automata and on their computational capabilities, with a special focus on the emergent behavioural properties of this new model and their significance in the context of computation-oriented interpretations of physical phenomena. A preliminary investigation of the relations between Nominal Cellular Automata and Wolfram's Elementary Cellular Automata is also carried out.

==> eptcsdata.tex <==
\providecommand{\firstpage}{24}
\providecommand{\publicationstatus}{M. Bartoletti, L. Henrio, S. Knight, and H. T. Vieira (Eds.):\\9th Interaction and Concurrency Experience (ICE 2016)\\
EPTCS 223, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.223.2}{10.4204/EPTCS.223.2}}
\pdfoutput=1

